Uncertainty Estimation for 3D Object Detection via Evidential Learning

3D object detection is an essential task for computer vision applications in autonomous vehicles and robotics. However, models often struggle to quantify detection reliability, leading to poor performance on unfamiliar scenes. We introduce a framework for quantifying uncertainty in 3D object detection by leveraging an evidential learning loss on Bird's Eye View representations in the 3D detector. These uncertainty estimates require minimal computational overhead and are generalizable across different architectures. We demonstrate both the efficacy and importance of these uncertainty estimates on identifying out-of-distribution scenes, poorly localized objects, and missing (false negative) detections; our framework consistently improves over baselines by 10-20% on average. Finally, we integrate this suite of tasks into a system where a 3D object detector auto-labels driving scenes and our uncertainty estimates verify label correctness before the labels are used to train a second model. Here, our uncertainty-driven verification results in a 1% improvement in mAP and a 1-2% improvement in NDS.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> fig/nu_pseudo_labelling_classwise_table.tex <==
\begin{table}[!t]
    \caption{{\bf nuScenes \ML{caption needs to be filled}} . }
    \label{tab:ood_results}  
    \scriptsize
    \centering
    \begin{tabular}{l c c c c c c c c c c c} \toprule
    & car & truck & bus & trailer & cv & pedestrian & motorcycle & bicycle & traffic\_cone & barrier & M\\
    \hline
    \textit{10k Labelled} & 0.848 & 0.555 & 0.671 & 0.354 & 0.202 & 0.854 & 0.686 & 0.497 & 0.647 & 0.567 & \multirow{7}{*}{\rotatebox{270}{FF (L)}} \\
    \textit{10k Pseudo} & 0.859 & 0.579 & 0.716 & 0.396 & 0.245 & 0.854 & 0.727 & 0.548 & 0.706 & 0.679 \\
    \textit{10k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Labelled} & 0.869 & 0.602 & 0.743 & 0.450 & 0.251 & 0.864 & 0.715 & 0.569 & 0.731 & 0.705 \\
    \textit{20k Pseudo} & 0.870 & 0.604 & 0.749 & 0.456 & 0.266 & 0.866 & 0.754 & 0.590 & 0.738 & 0.718 \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.873 & 0.591 & 0.762 & 0.444 & 0.282 & 0.873 & 0.757 & 0.608 & 0.742 & 0.703 \\ 
    \midrule
    \textit{10k Labelled} & 0.883 & 0.637 & 0.751 & 0.392 & 0.259 & 0.880 & 0.795 & 0.667 & 0.747 & 0.653 & \multirow{7}{*}{\rotatebox{270}{FF (L+C)}} \\
    \textit{10k Pseudo} & 0.885 & 0.634 & 0.757 & 0.394 & 0.285 & 0.871 & 0.816 & 0.693 & 0.763 & 0.679 \\
    \textit{10k Pseudo + Unc} & 0.885 & 0.633 & 0.756 & 0.394 & 0.288 & 0.873 & 0.820 & 0.689 & 0.768 & 0.690 \\
    \textit{20k Labelled} & 0.892 & 0.656 & 0.780 & 0.445 & 0.288 & 0.885 & 0.810 & 0.691 & 0.786 & 0.732 \\
    \textit{20k Pseudo} & 0.892 & 0.660 & 0.783 & 0.451 & 0.290 & 0.887 & 0.820 & 0.684 & 0.784 & 0.744 \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.894 & 0.654 & 0.788 & 0.456 & 0.305 & 0.887 & 0.830 & 0.709 & 0.795 & 0.732 \\
    \midrule
    \textit{10k Labelled} & 0.845 & 0.556 & 0.674 & 0.345 & 0.208 & 0.855 & 0.659 & 0.477 & 0.656 &  0.573 & \multirow{7}{*}{\rotatebox{270}{DF (L)}} \\
    \textit{10k Pseudo} & &  &  &  &  &  &  &  &  &  \\
    \textit{10k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Labelled} & 0.867 & 0.598 & 0.738 & 0.442 & 0.254 & 0.865 & 0.689 & 0.543 & 0.731 & 0.702 \\
    \textit{20k Pseudo} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.829 & 0.536 & 0.701 & 0.388 & 0.228 & 0.861 & 0.647 & 0.521 & 0.735 & 0.638 \\
    \bottomrule
    \end{tabular}
    % \vspace{-2mm}
%    \caption{\small {\bf nuScenes DeformFormer (Lidar only)}}
%    \label{tab:ood_results}  
\end{table}


==> fig/nu_pseudo_labelling_multiple_table.tex <==
\begin{table}[ht!]
    \caption{\small {\bf nuScenes FocalFormer (Lidar only)} . }
    \label{tab:ood_results}  
    \footnotesize
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
    & car & truck & bus & trailer & cv & pedestrian & motorcycle & bicycle & traffic\_cone & barrier \\
    \hline
    \textit{10k Labelled} & 0.848 & 0.555 & 0.671 & 0.354 & 0.202 & 0.854 & 0.686 & 0.497 & 0.647 & 0.567 \\
    \textit{10k Pseudo} & 0.859 & 0.579 & 0.716 & 0.396 & 0.245 & 0.854 & 0.727 & 0.548 & 0.706 & 0.679 \\
    \textit{10k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Labelled} & 0.869 & 0.602 & 0.743 & 0.450 & 0.251 & 0.864 & 0.715 & 0.569 & 0.731 & 0.705 \\
    \textit{20k Pseudo} & 0.870 & 0.604 & 0.749 & 0.456 & 0.266 & 0.866 & 0.754 & 0.590 & 0.738 & 0.718 \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.873 & 0.591 & 0.762 & 0.444 & 0.282 & 0.873 & 0.757 & 0.608 & 0.742 & 0.703 \\
    \hline
    \end{tabular}
    % \vspace{-2mm}
\end{table}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
    & car & truck & bus & trailer & cv & pedestrian & motorcycle & bicycle & traffic\_cone & barrier \\
    \hline
    \textit{10k Labelled} & 0.883 & 0.637 & 0.751 & 0.392 & 0.259 & 0.880 & 0.795 & 0.667 & 0.747 & 0.653 \\
    \textit{10k Pseudo} & 0.885 & 0.634 & 0.757 & 0.394 & 0.285 & 0.871 & 0.816 & 0.693 & 0.763 & 0.679 \\
    \textit{10k Pseudo + Unc} & 0.885 & 0.633 & 0.756 & 0.394 & 0.288 & 0.873 & 0.820 & 0.689 & 0.768 & 0.690 \\
    \textit{20k Labelled} & 0.892 & 0.656 & 0.780 & 0.445 & 0.288 & 0.885 & 0.810 & 0.691 & 0.786 & 0.732 \\
    \textit{20k Pseudo} & 0.892 & 0.660 & 0.783 & 0.451 & 0.290 & 0.887 & 0.820 & 0.684 & 0.784 & 0.744 \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.894 & 0.654 & 0.788 & 0.456 & 0.305 & 0.887 & 0.830 & 0.709 & 0.795 & 0.732 \\
    \hline
    \end{tabular}
    % \vspace{-2mm}
    \caption{\small {\bf nuScenes FocalFormer (Lidar + Camera only)} . }
    \label{tab:ood_results}  
\end{table}


\begin{table}[ht!]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
    & car & truck & bus & trailer & cv & pedestrian & motorcycle & bicycle & traffic\_cone & barrier \\
    \hline
    \textit{10k Labelled} & 0.845 & 0.556 & 0.674 & 0.345 & 0.208 & 0.855 & 0.659 & 0.477 & 0.656 &  0.573 \\
    \textit{10k Pseudo} & &  &  &  &  &  &  &  &  &  \\
    \textit{10k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Labelled} & 0.867 & 0.598 & 0.738 & 0.442 & 0.254 & 0.865 & 0.689 & 0.543 & 0.731 & 0.702 \\
    \textit{20k Pseudo} &  &  &  &  &  &  &  &  &  &  \\
    \textit{20k Pseudo + Unc} &  &  &  &  &  &  &  &  &  &  \\
    \textit{Full Training} & 0.829 & 0.536 & 0.701 & 0.388 & 0.228 & 0.861 & 0.647 & 0.521 & 0.735 & 0.638 \\
    \hline
    \end{tabular}
    % \vspace{-2mm}
    \caption{\small {\bf nuScenes DeformFormer (Lidar only)}}
    \label{tab:ood_results}  
\end{table}


==> fig/nuscenes_metrics_plot.tex <==
\begin{figure*}[htb]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.48\textwidth]{images/nuscenes_L.png} & \includegraphics[width=0.48\textwidth]{images/nuscenes_LC.png} \\ 
    \end{tabular}   
    \vspace{-2mm} 
    \caption{\small 
       {\bf Left.}  Accuracy of the lift-to-drag estimate as a function of the number of exemplars used to train the emulators. {\bf Right.}  Lift-to-drag ratio of the shapes during optimization, as a function of number of iterations. }
      \label{fig:comp}
\end{figure*}
